Matchings, Predictions and Counterfactual Harm in Refugee Resettlement Processes

Resettlement agencies have started to adopt data-driven algorithmic matching to match refugees to locations using employment rate as a measure of utility. Given a pool of refugees, data-driven algorithmic matching utilizes a classifier to predict the probability that each refugee would find employment at any given location. Then, it uses the predicted probabilities to estimate the expected utility of all possible placement decisions. Finally, it finds the placement decisions that maximize the predicted utility by solving a maximum weight bipartite matching problem. In this work, we argue that, using existing solutions, there may be pools of refugees for which data-driven algorithmic matching is (counterfactually) harmful -- it would have achieved lower utility than a given default policy used in the past, had it been used. Then, we develop a post-processing algorithm that, given placement decisions made by a default policy on a pool of refugees and their employment outcomes, solves an inverse~matching problem to minimally modify the predictions made by a given classifier. Under these modified predictions, the optimal matching policy that maximizes predicted utility on the pool is guaranteed to be not harmful. Further, we introduce a Transformer model that, given placement decisions made by a default policy on multiple pools of refugees and their employment outcomes, learns to modify the predictions made by a classifier so that the optimal matching policy that maximizes predicted utility under the modified predictions on an unseen pool of refugees is less likely to be harmful than under the original predictions. Experiments on simulated resettlement processes using synthetic refugee data created from a variety of publicly available data suggest that our methodology may be effective in making algorithmic placement decisions that are less likely to be harmful than existing solutions.

==> 011related.tex <==
%
\xhdr{Inverse Assignment Problems} Bipartite matching problems, or more generally assignment problems, have multifaceted applications in various domains and thus a rich, extensive literature \cite{gale1962college, crawford1981job, lovasz2009matching, gibbons1985algorithmic, stelmakh2021peer, mcelfresh2023matching, aziz2021optimal}. 
%
Less common and not well known are inverse assignment problems~\cite{demange2014introduction, heuberger2004inverse, lee2020inverse}. 
%
Whereas assignment problems aim to find an optimal assignment that maximizes a desired parameterized objective function, inverse assignment problems aim to find the minimal change to those parameters such that a desired assignment becomes an optimal assignment~\cite{liu2003inverse,berczi2023inverse}.
%
Inverse assignment problems have been recently proven useful in the context of counterfactual explanations~\cite{korikov2021counterfactual, korikov2021counterfactualconstraint}. In particular, finding the nearest counterfactual explanation for algorithmic assignments has been reduced to an inverse problem.
%
Within the literature on inverse assignment problems, 
%
the work most closely related to ours is
%
by Yang and Zhang~\cite{yang2007partial}, which introduces an algorithmic framework to solve partial inverse assignment problems 
%where the desired partial assignment is given.
where the desired assignment is only partially given.
%
More specifically, in our first methodological contribution, we adapt their framework 
to mi\-ni\-mally mo\-di\-fy the refugees' predicted employment probabilities by a given classifier (in their framework, the parameters) so that, 
%
under these modified probabilities, 
%
the optimal placement decisions (the optimal assignment) match a subset of those made by a default policy (the desired partial assignment).
% parameters such that all optimal matchings are guaranteed to contain the desired 
% partial matching.

\xhdr{Harm} The notion of harm plays an important role in many ethical principles of decision making~\cite{ross2011foundations, feinberg1984harm, mill1966liberty, smith2005origin, wright1985causation}. It constitutes an imperative part of what is considered a good action and how society judges decisions---one shall not cause harm to others.
%
What it means to cause harm is not unequivocally agreed upon; however, the most widely accepted definition is the counterfactual comparative account of harm~\cite{klocksiem2012defense, feinberg1986wrongful}.
%
Under this definition, an action is harmful to a person if and only if they would have been in a better state had the action not been taken.
%
Building upon this definition of harm, 
%
Richens et al.~\cite{richens2022counterfactual} have used the framework of probabilistic
structural causal models to argue that a reinforcement learning policy is harmful to a person if and only if they would have been in a better state had a default policy, presumably implemented by a human, been used.
%
In our work, we use this notion of harm in data-driven algorithmic matching.
% , rather than reinforcement learning.

% suhas: TBD -- include related work in final version \citep{li2023trustworthy}, \cite{beckers2022causal}
